Event-Based Motion Segmentation by Motion Compensation

In contrast to traditional cameras, whose pixels have a common exposure time, event-based cameras are novel bio-inspired sensors whose pixels work independently and asynchronously output intensity changes (called "events"), with microsecond resolution. Since events are caused by the apparent motion of objects, event-based cameras sample visual information based on the scene dynamics and are, therefore, a more natural fit than traditional cameras to acquire motion, especially at high speeds, where traditional cameras suffer from motion blur. However, distinguishing between events caused by different moving objects and by the camera's ego-motion is a challenging task. We present the first per-event segmentation method for splitting a scene into independently moving objects. Our method jointly estimates the event-object associations (i.e., segmentation) and the motion parameters of the objects (or the background) by maximization of an objective function, which builds upon recent results on event-based motion-compensation. We provide a thorough evaluation of our method on a public dataset, outperforming the state-of-the-art by as much as 10%. We also show the first quantitative evaluation of a segmentation algorithm for event cameras, yielding around 90% accuracy at 4 pixels relative displacement.

==> chapters/figures/fig_block_diagram.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/labelled_events/algorithm_process_reduced.png}
\vspace{-2ex}
   \caption{
   % Illustrate the solution, showing explicitly the ``layers'' and motion-compensated images.
   \emph{Event-based Motion Segmentation}.
   Events in a space-time volume $V$ on the image plane (Left) are the input to our clustering method, which infers the motion parameters of the clusters and the event-cluster association probabilities (Center).
   Events are clustered into objects with coherent motion, and are colored accordingly (Right).
   As a by-product, the method also provides motion-compensated (i.e., sharp) images of warped events; one for each cluster (Center).
   }
\label{fig:method:diagram}
\vspace{-1ex}
\end{figure*}

==> chapters/figures/fig_convergence_slices.tex <==
\begin{figure}[t]
    \centering
    \subfloat[Slice corresponding to motion parameters $\bparams_1$ of cluster 1 (a net undergoing a motion of \SI{280}{pixel/\second} horizontally)]{\includegraphics[width=0.48\linewidth]{images/experim/iros18/whatisbackground/data_plot_blur1_0.png}}~~
    \subfloat[Slice corresponding to motion parameters $\bparams_2$ of cluster 2 (a ball thrown at \SI{-450}{pixel/\second} horizontally)]{\includegraphics[width=0.48\linewidth]{images/experim/iros18/whatisbackground/data_plot_blur1_1.png}}
    \vspace{-1ex}
    \caption{Two 2-D slices of the objective function~\eqref{eq:weightedContrast} for the \seqwib\, sequence in Fig.~\ref{fig:scenes:Mitrokhin} (also, 1st row of Fig.~\ref{fig:allseqs}). 
    Close to convergence, the objective function is mostly determined by the motion parameters $\bparams=\{\bparams_1,\bparams_2\}$ that are the axes of these slices.
    \revred{But then, we did not use 4-DOF warpings... I would remove this plot}}
    \label{fig:whatisbackground:slices}
    \vspace{-2ex}
\end{figure}


==> chapters/figures/fig_n_motion_models.tex <==
\global\long\def\nmodelwidth{0.3\linewidth}
\begin{figure*}[t]
\centering
\subfloat[10x Optical Flow Clusters \label{fig:n_motion_models_vel}]{\frame{\includegraphics[width=\nmodelwidth]{images/n_motion_models/all_linvelocity/lin_velocity.png}}}~
\subfloat[5x Optical Flow/5x Rotation Clusters \label{fig:n_motion_models_half}]{\frame{\includegraphics[width=\nmodelwidth]{images/n_motion_models/half_and_half/half_and_half.png}}}~
\subfloat[10x Rotation Clusters \label{fig:n_motion_models_rot}]{\frame{\includegraphics[width=\nmodelwidth]{images/n_motion_models/all_rotation/rotation.png}}}
    \caption{\label{fig:n_motion_models} Scene from \cite{Mueggler17ijrr} segmented using our method with different mixtures of motion-model. Each cluster has its own color, evenly sampled from the color wheel.}
\end{figure*}


==> chapters/figures/tab_mitrokhin_comparison.tex <==
\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{lccc}
    \toprule
        \textbf{Sequence} & \textbf{SOFAS}~\cite{Stoffregen17acra} &\textbf{Mitrokhin}~\cite{Mitrokhin18iros} & \textbf{Ours (Alg.~\ref{alg:ems})} \\ \midrule
        {\small\texttt{Fast moving drone}} & 88.89 & 92.78 &  \textbf{96.30}\\
        {\small\texttt{Multiple objects}} & 46.15 & 87.32 &  \textbf{96.77}\\
        {\small\texttt{Lighting variation}} & 0.00 & \textbf{84.52} &  80.51\\
        {\small\texttt{What is Background?}} & 22.08 & 89.21 &  \textbf{100.00}\\
        {\small\texttt{Occluded sequence}} & 80.00 & 90.83 &  \textbf{92.31}\\ \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{
    Comparison with state-of-the-art.
    Success rate (in \si{\percent}) of detection of moving objects, as proposed by~\cite{Mitrokhin18iros}.
    }
    \label{tab:iros18}
\end{table}

